Communication-efficient Certificate Revocation Management for Advanced Metering Infrastructure and IoT

Advanced Metering Infrastructure forms a communication network for the collection of power data from smart meters in Smart Grid. As the communication between smart meters could be secured utilizing public-key cryptography, however, public-key cryptography still has certain challenges in terms of certificate revocation and management particularly related distribution and storage overhead of revoked certificates. To address this challenge, in this paper, we propose a novel revocation management approach by utilizing cryptographic accumulators which reduces the space requirements for revocation information significantly and thus enables efficient distribution of such information to all smart meters. We implemented the proposed approach on both ns-3 network simulator and a testbed. We demonstrated its superior performance with respect to traditional methods for revocation management.

==> Rebuttal/inputTable.tex <==
\begin{table}[]
\centering
\caption{\textcolor{red}{High-level Comparison of Revocation Management Schemes.}}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{{\color[HTML]{000000} }} &
  {\color[HTML]{FE0000} \textbf{Applicability}} &
  {\color[HTML]{FE0000} \textbf{\begin{tabular}[c]{@{}c@{}}Storage\\ Overhead\\Advantage\end{tabular}}} &
  {\color[HTML]{FE0000} \textbf{\begin{tabular}[c]{@{}c@{}}Communication\\
  Overhead\\Advantage\end{tabular}}} &
  {\color[HTML]{FE0000} \textbf{Security}} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{FE0000} OCSP}         & \Circle & \CIRCLE & \Circle & \CIRCLE \\
{\color[HTML]{FE0000} OCSP-Staple}  & \Circle & \CIRCLE & \Circle & \CIRCLE \\
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{FE0000} CRL}          & \LEFTcircle  & \Circle & \Circle & \CIRCLE \\
{\color[HTML]{FE0000} Delta CRL}    & \LEFTcircle & \CIRCLE & \LEFTcircle & \CIRCLE \\
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{FE0000} Bloom Filter} & \LEFTcircle & \CIRCLE & \LEFTcircle & \CIRCLE \\
{\color[HTML]{FE0000} Our Approach} & \CIRCLE & \CIRCLE & \CIRCLE & \CIRCLE \\
\bottomrule
\multicolumn{5}{c}{\small {\normalsize \CIRCLE} $=$ offers the benefit; {\normalsize \LEFTcircle} $=$ almost offers the benefit; no circle $=$ does not offer the benefit.} \\

\end{tabular}%
}
\end{table}
